Processing Natural Language on Embedded Devices: How Well Do Transformer Models Perform?

This paper presents a performance study of transformer language models under different hardware configurations and accuracy requirements and derives empirical observations about these resource/accuracy trade-offs. In particular, we study how the most commonly used BERT-based language models (viz., BERT, RoBERTa, DistilBERT, and TinyBERT) perform on embedded systems. We tested them on four off-the-shelf embedded platforms (Raspberry Pi, Jetson, UP2, and UDOO) with 2 GB and 4 GB memory (i.e., a total of eight hardware configurations) and four datasets (i.e., HuRIC, GoEmotion, CoNLL, WNUT17) running various NLP tasks. Our study finds that executing complex NLP tasks (such as "sentiment" classification) on embedded systems is feasible even without any GPUs (e.g., Raspberry Pi with 2 GB of RAM). Our findings can help designers understand the deployability and performance of transformer language models, especially those based on BERT architectures.

==> sections/Background_study.tex <==






\section{Backgrounds}
In this section, we first define our goal tasks (Sec. \ref{task}) and then, provide a brief background on transfer learning (Sec.\ref{subec:transfer_learn}), attention mechanism (Sec. \ref{subsec:attnhead}), and finally present an overview of BERT-based language models (Sec. \ref{subsec:Bert}).


\subsection{Goal Tasks}\label{task}

As mentioned in Sec.~\ref{introduction}, two pivotal tasks associated with user utterance understanding are \textit{Intent Classification} (IC)  and \textit{Named Entity Recognition} (NER), which we exclusively focus on in this paper. For example, consider the following user utterance: 
 
\enquote{\textit{Bring the book from the table}} 
 
This utterance expresses that the user instructed the assistant to \enquote{Bring} something and thus, the user intent here is identified as ``Bring''. Automatic identification of such intents is defined as the \textit{Intent Classification} task. Now, the questions are what will the assistant bring? and from where? By looking at the simple utterance, as humans, we know that the answers to the first and second questions are \enquote{book} and \enquote{table}, respectively. Both \enquote{book} and \enquote{table} are entities and need to be identified by the robot properly in order to execute the ``bring'' action. Automatic identification and extraction of such entities are defined as the  \textit{Named Entity Recognition} task. We provide further details on these two tasks in section \ref{problem_statement}.




\subsection{Transfer Learning}\label{subec:transfer_learn}
Transfer learning is a machine learning paradigm where a model trained for one task/problem is reused as the starting point to further train the model on a different task (or problem). Broadly, transfer learning can be performed in two steps, \textit{Pretraining} and \textit{Finetuning}. For an instance, given an NLP model $M$, datasets/tasks $A$ and $B$, transfer learning is performed in the following steps:

\begin{enumerate}
    \item Train $M$ using dataset $A$.
    \item Keep some/all of the learned parameters of $M$ unaltered.
    \item Further train $M$ using dataset $B$.
\end{enumerate}

Here, step 1 is called the pretraining phase of \textit{Transfer Learning}. Whereas steps 2 and 3 are called the "finetuning phase" where the model is customized for a different dataset. There are significant benefits to using such a pretraining/finetuning paradigm. It reduces computation costs and allows us to reuse previous computations without having to train a new model from scratch. Due to the large size of existing language models with millions of parameters and the long time required to train them from scratch, pretraining them on a large corpus once followed by fine-tuning on many small, task-specific corpora has become a standard practice within the ML/NLP community. Notably, BERT (refer to section \ref{subsec:Bert}) is pretrained on Masked Language Model (MLM) and Next Sentence Prediction (NSP) tasks~\cite{bert}. Finetuning of BERT is a straightforward step \cite{bert} which is usually done by adding a dense outer layer on top of the pretrained BERT model and then training on the task-specific dataset.



\subsection{Attention Mechanism}\label{subsec:attnhead}
Attention is a powerful and ubiquitous mechanism for allowing deep neural models to focus on particular salient pieces of information by taking their weighted average when making predictions~\cite{vaswani2017attention}. An attention mechanism lets each token from the input sequence (e.g. sentences made of word or sub-word tokens) focus on other specific tokens. Say the following sentence is an input sentence for an NLP task:

\enquote{\textit{The animal didn't cross the street because it was too tired}.}

What does \enquote{it} in this sentence refer to? Is it referring to the street or to the animal? It’s a simple question for a human, but not as simple for a machine. When the machine is processing the word "it", attention allows it to associate "it" with "animal".
As the model processes each word (each position in the input sequence), attention allows it to look at other positions in the input sequence for clues that can lead to a better understanding of context.



\subsection{BERT}\label{subsec:Bert}

The Transformer~\cite{vaswani2017attention} is a deep learning architecture that aims to solve sequence-to-sequence tasks while handling long-range dependencies with ease. It relies on self-attention and positional encoding to compute representations of its input and output without using recurrent or convolutional neural networks. Transformer-based networks trained with large multi-domain datasets have unlocked a series of breakthroughs in natural language processing. A major catalyst of this success is the Bidirectional Encoder Representations from the Transformers technique, or Google’s BERT~\cite{bert}. BERT framework learns information from both the right and left sides of a word (or token). This makes it more powerful at understanding context.
A pre-trained BERT model is remarkably easy to adapt to different NLP applications. It can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. \hl{In our experiments, we used $BERT_{Base}$ which has 12 layers of transformers block with a hidden size of $768$ and number of self-attention heads as 12 and has around 110M trainable parameters.}


